Nearly Optimal Private Convolution

We study computing the convolution of a private input $x$ with a public input $h$, while satisfying the guarantees of $(\epsilon, \delta)$-differential privacy. Convolution is a fundamental operation, intimately related to Fourier Transforms. In our setting, the private input may represent a time series of sensitive events or a histogram of a database of confidential personal information. Convolution then captures important primitives including linear filtering, which is an essential tool in time series analysis, and aggregation queries on projections of the data. We give a nearly optimal algorithm for computing convolutions while satisfying $(\epsilon, \delta)$-differential privacy. Surprisingly, we follow the simple strategy of adding independent Laplacian noise to each Fourier coefficient and bounding the privacy loss using the composition theorem of Dwork, Rothblum, and Vadhan. We derive a closed form expression for the optimal noise to add to each Fourier coefficient using convex programming duality. Our algorithm is very efficient -- it is essentially no more computationally expensive than a Fast Fourier Transform. To prove near optimality, we use the recent discrepancy lowerbounds of Muthukrishnan and Nikolov and derive a spectral lower bound using a characterization of discrepancy in terms of determinants.

==> Conclusion__S_muthukrishnan_s_conflicted_copy_2012-12-05_.tex <==
\section{Conclusion} 

We derive nearly tight upper and lower bounds on the error of $(\eps,
\delta)$-differentially private for computing convolutions. Our lower
bounds rely on recent general lower bounds based on discrepancy theory
and elementary linear algebra; our upper bound is a simple
computationally efficient algorithm. We also sketch several
applications of private convolutions, in time series analysis and in
computing generalizes marginal queries on a $d$-attribute database.

Our results are nearly optimal for any $h$ when the database size is
large enough with respect to the number of queries. In some settings
it is reasonable to assume however that database size is much smaller,
and our algorithms give suboptimal error for such sparse
databases. Nearly optimal algorithms for  computing a workload of $M$ linear queries
posed to a  database of size at most $n$ were given
in~\cite{geometry}, but their algorithm has running time at least
$O(M^2Nn)$. Since our dense case algorithm for computing convolutions
has running time $O(N \log N)$, an interesting open problem is to give
an algorithm with running time $O(Nn \polylog(N,n))$ for computing
convolutions with optimal error when the database size is at most
$n$. 

\junk{
Note: Subsequently to our work,  quite recently, our results were generalized
by Nikolov, Talwar, and Zhang~\cite{geometry} to give instance-optimal
$(\eps, \delta)$-differentially a private algorithm for any workload
of linear queries. However, the generality of their result comes at a
cost in efficiency: their algorithm needs to compute a minimum
enclosing ellipsoid of a convex body and has running time at least
$O(M^2N)$. 
}


==> Conjecture.tex <==
\section{Conjecture}

the conjecture

why it is wrong: 

http://mathoverflow.net/questions/83208/an-approximate-converse-of-discrete-uncertainty-principle 


how we can turn it into a lower bound
from our email:

1)      Are you sure the conjecture you state is the correct one, given the normalization issues we discussed before you left, meaning the factor $ \sqrt (n) in \hat{H}$ ?

Yupp. The conjecture didn't change. We actually changed $\hat{H}$ to go with the normalization used in the conjecture.

2)      Can we find interesting functions for which this holds and that one would like to be private? (same question as in email below)

One answer is "compressible" functions we've been talking about. Intuitively we probably should expect functions which are somehow periodic to be compressed in the frequency domain.

3)      If this concentration property is an exception rather than the norm, how come your simulations showed it to be true for all $n <23$? What did you simulate exactly?

Good question. Either I did something wrong or there is an asymptotics issue going on: the concentration fails for higher n maybe. I simply enumerated over all h $\in {0, 1}^n$ and tested the conjecture.

4)      If this concentration is not the norm, but rather the spreading out, can we use this to show a lower bound on the noise for diff privacy for general convolution functions?

That's a good question too. Maybe, using the eigenvalue approach to lower bounds that I showed you.


==> DNF.tex <==
\subsection{Convolution over Abelian Groups and Applications}

\textbf{Convolution over Abelian Groups.} The circular convolution
defined above is a special case of the more general concept of
convolution over finite abelian groups. Let $G$ be an abelian group
and let $x:G \rightarrow \C$ and $h:G \rightarrow \C$ be functions
mapping $G$ to the complex numbers. We define the convolution $x \ast
h:G \rightarrow \C$ of $x$ and $h$ as:
\begin{equation*}
  (x \ast h)(a) = \sum_{a \in G}{x(b)h(a-b)}
\end{equation*}
In the above equation the operation $a - b$ is done in the group
$G$. Circular convolution can be thought as the case when $G$ is the
additive group $\mathbb{Z}/N\Z$ of integers modulo $N$ and the the
sequences $x$ and $h$ encode functions from $\Z/N\Z$ to $\C$. Similarly,
we can think of $x$ and $h$ above as sequences of length $|G|$ indexed
by elemengs of $G$, where $x_a$ is an equivalent notation for $x(a)$.

This more general form of convolution shares most important properties
of circular convolution: it is commutative and linear in both $x$ and
$h$; also $x \ast h$ can be diagonalized by an appropriately defined
Fourier basis which reduces $\bF_N$ as defined above in the case of
$\Z/N$. In particular, $x \ast h$ (as say a linear operator on $x$) is
diagonalized by the irreducible characters of $G$, which can be
indexed by elements of $G$, and also the corresponding Fourier
coefficients are indexed by elements of $x$.

We note that all our results carry over to the general case of
convolution over abelian groups, as we do not rely in any way on the
structure of $\Z/N\Z$. The properties of the Fourier transform that we
use are: \textbf{(1)} it diagonalizes the convolution operator;
\textbf{(2)} any component of any Fourier basis vector has unit
norm. Both these properties hold in the general case. In any theorem
statement, the private sequence $x$ and the public sequence $h$ can be
thought of as a functions; the parameter $N$ can be substituted by
$|G|$ and Fourier coefficients can be indexed by elements of $G$
instead of the numbers $0, \ldots, N-1$.

Of particular interest for us is the case $G = (\Z/2\Z)^d$,
i.e.~boolean functions. In that case each element $a$ of $G$ can be
represented as a 0-1 sequence $a_1, \ldots, a_d$, and also as a set $S
\subseteq [d]$ for which $a$ is an indicator. Characters are then
indexed by sets $S \subseteq [d]$ and are functions $\chi_S:G
\rightarrow \C$ defined by
\begin{equation*}
  \chi_S(a) = \frac{1}{2^{d/2}}\prod_{i \in S}{(-1)^{a_i}}.
\end{equation*}
Fourier coefficients of a function $g:G \rightarrow \C$ are also
indexed by sets $S \subseteq [d]$; the coefficient of $g$
corresponding  to $\chi_S$ is denoted $\hat{g}(S)$.

\textbf{Generalized Marginal Queries.}
Some aggregation operations on databases with $d$ binary attributes
can be naturally expressed as convolutions over $(\Z/2)^d$. Consider a
private database $D$, modelled as a multiset of $n$ binary strings in
$\{0, 1\}^d$, i.e.~$D \in (\{0, 1\}^d)^n$. Each element of $D$
corresponds to a user whose data consists of the values of $d$ binary
attributes: the $i$-th bit in the binary string of a user is the value
of the $i$-th attribute for that user. The database $D$ can be
represented as a sequence $x$ of length $2^d$ or equivalently as a
function $x:\{0, 1\}^d \rightarrow [n]$, where for $a \in \{0, 1\}^d$,
$x(a)$ is the number of users whose attributes are specified by $a$
(i.e.~the number of occurances of $a$ in $D$). Note that $x$ can be
thought of as a function from $(\Z/2\Z)^d \rightarrow [n]$. Note also
that removing or adding a single element to $D$ changes $x$ (thought of as a
vector) by at most $1$ in the $\ell_1$ norm.

Consider a convolution $x \ast h$ of the database  $x$ with a
binary function $h:(\Z/2\Z)^d \rightarrow \{0, 1\}$. Let
$\mathbf{1}\{a_i \neq b_i\}$ be an indicator of the relation $a_i \neq
b_i$. Then $x \ast h$ represents the following aggregation
\begin{equation*}
  (x \ast h)(a) = \sum_{b \in \{0, 1\}^d}{x(b)h(\mathbf{1}\{a_1 \neq
    b_1\}, \ldots, \mathbf{1}\{a_d \neq b_d\})}.
\end{equation*}
A class of functions $h$ that has received much attention in the
differential privacy literature is the class of conjunctions. In that
case, $h$ is specified by a set $S \subseteq [d]$ of size $w$ and
$h(c) = 1$ if and only if $c_i = 0$ for all $i \in S$. Thus, $h(c) =
\bigwedge_{i \in S}{\bar{c_i}}$. For any such $h$, the convolution $x
\ast h$ evaluated at $a$ gives a $w$-way marginal: for how many users
do the attributes corresponding to the set $S$ equal the corresponding
values in $a$. The full sequence $x \ast h$ gives all marginals for
the set $S$ of attributes. This model was first studied in private
data analysis by Barak et al.~\cite{barak2007privacy} and has led to
an expanding line of work~\cite{kasiviswanathan2010price,gupta2011privately,hardt2012private}.

Here we define a generalization of marginals that allows $h$ to be not
only a conjunction of $w$ literals, but an arbitrary $w$-DNF.

\begin{definition}
  Let $h(c)$ be a $w$-DNF given by $h(c) = (\ell_{1, 1}
  \wedge \ldots \wedge \ell_{1,w}) \vee \ldots \vee (\ell_{s, 1}
  \wedge \ldots \wedge \ell_{s, w})$, where $\ell_{i, j}$ is a
  literal, i.e.~either $c_p$ or $\bar{c_p}$ for some $p \in [d]$. The
  generalized marginal function for $h$ and a database $x:\{0, 1\}^d
  \rightarrow [n]$ is a function $(x \ast h):\{0, 1\}^d \rightarrow
  [n]$ defined by
  \begin{equation*}
    (x \ast h)(a) = \sum_{b \in \{0, 1\}^d}{x(b)h(\mathbf{1}\{a_1 \neq
    b_1\}, \ldots, \mathbf{1}\{a_d \neq b_d\})}.
  \end{equation*}
\end{definition}

The overload of notation for $x \ast h$ here is on purpose as the
generalized marginal is indeed the convolution of $x$ and $h$ over the
group $(\Z/2\Z)^d$.

While marginals give, for each setting of attributes $a$, the number
of users whose attributes agree with $a$ on some $S$, generalized
marginals allow more complex queries such as, for example, ``show all
users who agree with $a$ on $a_1$ and at least one other
attribute''. Interestingly, our error bounds will depend only on the
width $w$ of the DNF $h$ and not on its size $s$. Previous work by
Barak et al.~\cite{barak2007privacy} relied on the fact that
conjunctions of $w$ literals, for $w$ much smaller than $d$, have
relatively few nonzero Fourier coefficients. In our work, we rely on
the fact that functions specified by $w$-DNF formulas have \emph{most}
of their weight concentrated on a few Fourier coefficients. This is a
challenge, as even small coefficients cannot be completely ignored in computing
the convolution. Nevertheless, our almost optimal algorithm for computing
convolutions exploits sparsity in the Fourier domain by calibrating
the noise according to the magnitude of Fourier coefficients. 

==> InputPerturbation.tex <==
\subsection{Input Perturbation}


\begin{theorem}[$IPT$]\label{thm:IPT}
Consider the linear map $\by=\bA \bx$, where $\bA \in \R^{M \times N}$.
Suppose that algorithm $\alg_{IPT}$ first adds noise to the input in the time domain: $\tilde{\bx}= \bx + \bz$, where $\bz$ is sampled from $\alpha_{q, \eps, \|\bI_N \|_{p,q}}(\R^N)\mu_{q, \eps, \|\bI_N \|_{p,q}}(\vec{z})$, and then outputs   $\tilde{\by}= \bA \tilde{\bx}$.
Then $\alg_{IPT}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, unbiased and it achieves MSE on the $m$-th component
\begin{equation}\label{eq:MSE_IPT}
\sigma_{z_m}^2=
\left\{
\begin{array}{ll}
 2 \frac{\| \bA_{m :} \|_2^2}{\eps^2} & \mbox{ if } p=1  \\
 \left(1 + \frac{1}{M} \right) \frac{M }{\eps^2} \| \bA_{m :} \|_2^2  & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
\end{theorem}

\begin{proof}
$\tilde{\bx}= \bx + \bz$ is $(\eps,0)$-differentially private by Theorem~\ref{th:eps0-DiffPriv} and Lemma~\ref{lm:spqSensitivity}, and consequently, $\tilde{\by}=\bA \tilde{\bx}$ is also $(\eps,0)$-differentially private by Theorem~\ref{thm:simple-composition}.

%Input perturbation in the time domain by additive noise
%\begin{equation}
%\begin{split}
%\tilde{\bx}&= \bx + \bz' \\
%\tilde{\by}&= \bA \tilde{\bx} = \bA  \bx + \bA \bz' = \by + \bz,
%\end{split}
%\end{equation}
%where $\bz'$ is a random noise vector in $\R^N$.
%%
%If $\bz'$ is sampled with probability density $\alpha_{q, \eps, \|\bI_N \|_{p,q}}(\R^N)\mu_{q, \eps, \|\bI_N \|_{p,q}}(\vec{z})$, then by Theorem~\ref{th:eps0-DiffPriv}, $\tilde{\bx}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, and consequently, $\tilde{\by}$ is also $(\eps,0)$-differentially private by Lemma~\ref{}.

The noise $\bz$ has mean zero. Note that $\|\bI_N\|_1 =\|\bI_N\|_2 = \|\bI_N\|_{\infty}=1$, thus its covariance matrix is
\begin{equation}
\E [\bz \bz^T]=
\left\{
\begin{array}{lll}
 2 \frac{1}{\eps^2} \bI_N & \mbox{ if } p=1 & \mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
 \left(1 + \frac{1}{N} \right) \frac{N }{\eps^2} \bI_N  & \mbox{ if } p=2 & \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
\end{array}
\right.
\end{equation}
%
%\begin{equation}
%\sigma_z'^2= \E [|z'_n|^2]=
%\left\{
%\begin{array}{lll}
% 2 \frac{1}{\eps^2}  & \mbox{ if } p=1 & \mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
% \frac{N }{\eps^2} \left(1 + \frac{1}{N} \right)   & \mbox{ if } p=2 & \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
%\end{array}
%\right.
%\end{equation}
%
The output of $\alg_{IPT}$ is $\tilde{\by}= \by + \bA \bz$. The final noise $\bz'=\bA \bz$ has mean 0. Observing that each component $z'_m = \bA_{m :} \bz$ has variance $\sigma_{z_n}^2=  \bA_{m :} \E[\bz \bz^T] \bA_{m :}^T$ gives Eq. (\ref{eq:MSE_IPT}).
\end{proof}

\begin{cor}
Consider the circular convolution $\bH \in \R^{N \times N}$ {\rm (\ref{eq:circConv})}. The algorithm $\alg_{IPT}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{ll}
2 \frac{\| \bh \|_2^2}{\eps^2} & \mbox{ if } p=1 \\
 \left(1 + \frac{1}{N} \right) \frac{N }{\eps^2} \| \bh \|_2^2  & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
\end{cor}

Note that
$
\frac{\|\bh\|_2^2}{\eps^2}
\leq \frac{\|\bh\|_1^2}{\eps^2}
\leq N \frac{\|\bh\|_2^2}{\eps^2}
\leq  N^2 \frac{\max_{m} |\hat{h}_m|^2}{\eps^2}
\leq  N\frac{\|\bh\|_1^2 }{\eps^2}.
$
The first (resp. third) inequality implies that input perturbation requires less noise for $\ell_1$ (resp. $\ell_2$) neighbors than output perturbation in the time domain.

%------------------------------
% $(\eps,delta)$- diff privacy
%------------------------------

\begin{theorem}[$\delta-IPT$]\label{thm:deltaIPT}
Consider the linear map $\by=\bA \bx$, where $\bA \in \R^{M \times N}$.
Suppose that algorithm $\alg_{\delta IPT}$ first adds noise to the input in the time domain: $\tilde{\bx}= \bx + \bz$, where $\bz$ is sampled from $\Lap\left(0, \frac{\sqrt{2M \ln (1/\delta)}}{\eps}\right)^M$, and then outputs   $\tilde{\by}= \bA \tilde{\bx}$.
Then $\alg_{\delta IPT}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors, unbiased and it achieves MSE on the $m$-th component
\begin{equation}\label{eq:MSE_deltaIPT}
\sigma_{z}^2=
 4 M \frac{\| \bA_{m :} \|_2^2}{\eps^2} \ln \left( \frac{1}{\delta} \right)
\end{equation}
\end{theorem}

\begin{cor}
Consider the circular convolution $\bH \in \R^{N \times N}$ {\rm (\ref{eq:circConv})}. The algorithm $\alg_{\delta IPT}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE 
\begin{equation}\label{eq:MSE_deltaIPT-Conv}
\sigma_{z}^2=
 4 N \frac{\| \bh \|_2^2}{\eps^2} \ln \left( \frac{1}{\delta} \right)
\end{equation}
 
\end{cor}

==> Intro-SigProcNad.tex <==
\section{Introduction}

\subsection{Motivations}

Why considering convolution?

Applications

\begin{itemize}
\item Dynamic binary/windowed/decayed sums = particular cases of convolution

\item Convolution: efficiently represented in Fourier Domain (~diagonal matrix) and DFT can be computed efficiently

\item \textbf{Signal processing}


Refs:

- \url{https://engineering.purdue.edu/~ee538/DFTbasedLinearFiltering.pdf}
Section 7.3: "DFT based linear filtering"  of the book " Introduction to Digital Signal Processing: Principles, Algorithms and Applications" by Proakis

- \url{http://www.ingelec.uns.edu.ar/pds2803/Materiales/LibrosPDF/Oppenheim/booktext08.pdf}
Chapter 8, "the discrete Fourier transform", of the book "Discrete-Time Signal Processing" by Oppenheim and Schafer

%\begin{itemize}
%
%\item

Linear time invariant (LTI) systems, such as linear filters of signals, (e.g. speech waveform filtering, audio or image compression), can be implemented by linear convolution \cite{Oppenheim-1989,Proakis-1992}.
Consider a discrete-time signal $x_n$, for example obtained by sampling a continuous-time speech waveform $x(t)$.
An input signal $x_n$ fed into an LTI filter with impulse response $h_n$, yields a filtered output signal $y=x \ast h$, where $\ast$ denotes the linear convolution of two sequences: $y_k=\sum_{n=-\infty}^{\infty} x_n h_{k-n}$.
Equivalently in the frequency domain, the discrete-time Fourier transform (DTFT) of the input $X(f)=\sum_{n=-\infty}^{\infty} x_n e^{-j 2 \pi f n}$, and the DTFTs $Y(f)$ and $H(f)$ of the output and of the filter response are related by $Y(f)=H(f)X(f)$.
For example, a filter response with a small gain at a particular frequency $f$ will suppress this frequency from the input signal. This property is used for example in low-pass filters, such as the ideal low pass filter with frequency response $H(f)=1$ if $ |f| < f_c$, $0$ otherwise, which selects frequencies below a cut-off frequency $f_c$, and cuts higher frequencies.

The DTFT is a function of a continuous variable $f$, thus its computation cannot be performed by a digital computer. However, for finite duration signals, $x_n$, $n\in\{0,\ldots,N-1\}$, there exists an alternative Fourier representation, namely the discrete Fourier transform (DFT), defined as $\hat{x}_m = \sum_{n=0}^{N-1} x_n e^{-j \frac{2 \pi m n}{N} }$, for $m\in\{0,\ldots,N-1\}$.
Note that the DFT is a sequence, rather than a function of the continuous variable $f$. In particular, the $m$-th element $\hat{x}_m$ of the DFT sequence is the $m$-th sample of the DTFT $X(f)$ at frequency $1/N$: $\hat{x}_m=X(m/N)$. A digital computer can perform the entry-wise product of the DFTs $\hat{x}$ and $\hat{h}$ of two sequences $x$ and $h$: $\hat{y}_m=\hat{x}_m\hat{h}_m $.
However, taking the inverse DFT (IDFT) of the sequence $\hat{y}_m$ yields the circular convolution of the sequences $x_n$ and $h_n$ in the time domain: $y'_k =  \sum_{n=0}^{N-1} x_n h_{(k-n)[N]}$, rather than the linear convolution $y_k =  \sum_{n=0}^{N-1} x_n h_{k-n}$ which represents linear filtering. Nevertheless, the linear convolution of finite duration sequences can be emulated by their circular convolution through zero-padding methods  \cite{Oppenheim-1989,Proakis-1992}.
Finally, it should be pointed out that there exist efficient algorithms ($N \log N$ complexity), named Fast Fourier Transform (FFT) algorithms, to compute the DFT of a finite duration sequence.

In summary, linear filtering can be performed as a linear convolution. Linear convolution can be emulated by circular convolution, through zero-padding methods \cite{Oppenheim-1989,Proakis-1992}. The circular convolution of two sequences can be efficiently performed as the entry-wise multiplications of their DFTs. DFT can be efficiently computed by FFT algorithms.
    In other words, if one wants to process a discrete-time signal $x$ by a linear time-invariant filter $h$ through the linear convolution $y=h\ast x$, it is more efficient computationally to do step 1-4 below than to directly compute the convolution.
\begin{enumerate}
\item pad $x$ and $h$ with zeros
\item compute the DFTs of the padded $x$ and $h$
\item multiply entry-wise these DFTs to obtain $\hat{y}$ (circular convolution computed in the Fourier domain)
\item take the inverse DFT of $\hat{y}$ to obtain the filtered y (result of the circular convolution in the time domain, emulating the linear convolution)
\end{enumerate}
This is the reason why in this paper, we focus on the circular convolution of two sequences.

%\item The circular convolution of two sequences can be efficiently performed as the entry-wise multiplications of their DFTs. discrete Fourier transforms (DFT): the product in the Fourier domain of the DFTs $\hat(x)$ and $\hat(h)$ of two sequences $x$ and $h$ corresponds, in the time domain (by Inverse DFT), to the circular convolution of the two sequences.
%
%\item  There exist efficient algorithms ($N \log N$ complexity), named Fast Fourier Transform (FFT) algorithms, to compute the DFT of a finite duration sequence.
%
%
%\end{itemize}
%
%In summary, if one wants to process a discrete-time signal $x$ by a linear time-invariant filter $h$ through the linear convolution $y=h\ast x$, it is more efficient computationally to do step 1-4 below than to directly compute the convolution.
%\begin{enumerate}
%\item pad $x$ and $h$ with zeros
%\item compute the DFTs of the padded $x$ and $h$
%\item multiply entry-wise these DFTs to obtain $\hat{y}$ (circular convolution computed in the Fourier domain)
%\item take the inverse DFT of $\hat{y}$ to obtain the filtered y (result of the circular convolution in the time domain, emulating the linear convolution)
%\end{enumerate}







\item Connection with some prior work on k-way marginals.









For the k-way marginals setting, we think of each row of the database as an element of $\{0, 1\}^d$,  i.e., each user has $d$ binary attributes, for example the attributes can be "Male?", "Married", "Lives in CA?" (in this case $d = 3$). We can write the database as a "histogram": a function $f : \{0, 1\}^d \rightarrow \R$, where $f(x_1, ..., x_d)$ gives the number of users with attribute values $x_1, \ldots, x_d$.  In our example $f(0, 1, 1)$ will be the number of married women living in CA.

A k-way marginal is given by a set $S \subset [d]$, $|S| = k$ and is a function $g_S : \{0, 1\}^S \rightarrow \R$. For each setting of the k attributes in $S$, $g_S$ gives the total number of users in the database that have the corresponding attribute values. For the example, a 2-way marginal is $g_{1, 3}(1, 1)$ which gives the number of men (both married and unmarried) living in CA.

There is some prior work in \url{http://research.microsoft.com/pubs/64344/contingency.pdf} that uses the Fourier transform to compute k-way marginals with less error than the naive approach (and to achieve consistent marginals). I was aware of that but I was not realizing that they actually compute a convolution and the function they are convolving with is sparse. What I mean is:

\begin{itemize}
\item We can extend $g_S$ from the domain $\{0, 1\}^S$ to the domain $\{0, 1\}^d$ in the natural way: components not in $S$ are just ignored (this is more for technical reasons); for example, above we can write $g_{1, 3}(1, 0, 1) = g_{1, 3}(1, 1, 1) = g_{1, 3}(1, 1)$
\item Then we can write $g_S$ as a convolution of $f$ and a function $h_S:\{0, 1\}^d \rightarrow \R$. We define $h_S$ as $h_S(x) = 1$ if and only if $x_i = 0 \:\: \forall i \in S$. The convolution is in the group $(\Z_2)^d$: $(f * h)(x) \triangleq \sum_{z \in \Z_2^d} { f(y + z \mod 2)h(z) }$ (as opposed to $\Z_n$ which is what we have been thinking about, but that does not affect any of the math). We have $(f * h_S)(x) = \sum_{y \mbox{ agrees with} x \mbox{ on } S}{ f(y) }$
\item The function $h_S$ has only $2^k$ nonzero Fourier coefficients (out of $2^d$ total).
\end{itemize}

So, the results in Barak et al. are a special case of computing convolutions of a private function/vector and a public function/vector which is sparse in the Fourier basis.

It seems that in their work, looking at the Fourier basis helps only with $\eps$-differential privacy, but not with $(\eps, \delta)$-d.p. It also seems to help make the marginals consistent.

But I still think it will be interesting to look at functions $h: \Z_2^d \rightarrow \{0, 1\}$ which are approximately sparse in the Fourier domain and see if convolutions $f * h$ for such functions are meaningful/interesting. Might lead to nice applications.


There is work, esp. in learning theory, on analyzing the fourier spectrum of functions $h:\{0, 1\}^d \rightarrow \{0, 1\}$ and proving that certain interesting examples have most of their weight concentrated on a few fourier coefficients (so they are approximately sparse as opposed to exactly sparse, like in Barak et al.). Here the fourier transform I am talking about is the one for $(\Z_2)^d$.


\end{itemize}





Challenge

Can applying differential privacy in the Fourier domain, rather than the time domain, result in an improved privacy-accuracy trade-off?








\subsection{Contributions}


Ongoing work

Randomized response, output perturbation in the time domain, and output perturbation in the Fourier domain: No gain so far
	$\Rightarrow$ noise variance scales with energy of the convolution filter impulse response

Investigating assumptions on convolution filer impulse response (e.g. compressibility) to obtain improved privacy-accuracy trade-off

\begin{table}\label{tab:MSEcomparison}
\begin{tabular}{| l || c | c | c |}
\hline
                                    & \textbf{Linear map $\bA$}  & \textbf{Convolution $\bH$}  & \textbf{p-Compressible Convolution }  \\ \hline \hline
\textbf{UB Output Pert. in time}    &                            &                             &                                     \\ \hline
\textbf{UB  Output Pert. in freq.}  &                            &                             &                                     \\ \hline
\textbf{UB  Input Pert.}            &                            &                             &                                     \\ \hline
\textbf{UB  Iterative algo}         &                            &                             &                                     \\ \hline
\textbf{LB  }                       &                            &                             &                                     \\
\hline
\end{tabular}
\caption{Mean square error for $\ell_1$ neighbors}
\end{table}


    


\subsection{Prior Work}

Optimizing Linear Counting Queries Under Differential Privacy

http://www.cs.cornell.edu/~mhay/papers/li2010optimizing.pdf

On the Geometry of Differential Privacy

http://research.microsoft.com/apps/pubs/default.aspx?id=119027.

Alex: I am wondering if their results imply that their K-norm mechanism gives optimal bounds for total l2 noise for epsilon-d.p. algorithms (assuming the slicing conjecture).

Haitham Hassanieh, Piotr Indyk, Dina Katabi, and Eric Price "Simple and Practical Algorithm for Sparse Fourier Transform," SODA, 2012.

http://nms.lcs.mit.edu/~dina/pub/soda12.pdf



==> Intro.tex <==
\section{Introduction}

\subsection{Motivations}

Why considering convolution?

Applications

\begin{itemize}
\item Dynamic binary/windowed/decayed sums, and more generally weighted moving averages = particular cases of convolution

\item Convolution: efficiently represented in Fourier Domain (~diagonal matrix) and DFT can be computed efficiently

\item \textbf{Linear filtering for financial analysis and signal processing}


%Refs:
%
%- \url{https://engineering.purdue.edu/~ee538/DFTbasedLinearFiltering.pdf}
%Section 7.3: "DFT based linear filtering"  of the book " Introduction to Digital Signal Processing: Principles, Algorithms and Applications" by Proakis
%
%- \url{http://www.ingelec.uns.edu.ar/pds2803/Materiales/LibrosPDF/Oppenheim/booktext08.pdf}
%Chapter 8, "the discrete Fourier transform", of the book "Discrete-Time Signal Processing" by Oppenheim and Schafer


Linear time invariant (LTI) filters, such as linear filters used in financial analysis \cite[Chapter 2]{Gencay-2002} (e.g. moving averages of financial time series) or signal processing (e.g. speech waveform filtering, audio or image compression, correlation function computation) \cite[Chapter 8]{Oppenheim-1999},\cite[Chapter 7]{Proakis-1992}, can be implemented by linear convolution.

Consider a discrete-time signal $x_n$, for example obtained by sampling a continuous-time speech waveform $x(t)$.
An input signal $x_n$ fed into an LTI filter with impulse response $h_n$, yields a filtered output signal $y=x \ast h$, where $\ast$ denotes the linear convolution of two sequences: $y_k=\sum_{n=-\infty}^{\infty} x_n h_{k-n}$.
Equivalently in the frequency domain, the discrete-time Fourier transform (DTFT) of the input $X(f)=\sum_{n=-\infty}^{\infty} x_n e^{-j 2 \pi f n}$, and the DTFTs $Y(f)$ and $H(f)$ of the output and of the filter response are related by $Y(f)=H(f)X(f)$.
For example, a filter response with a small gain at a particular frequency $f$ will suppress this frequency from the input signal. This property is used for example in signal processing to design low-pass filters, such as the ideal low pass filter with frequency response $H(f)=1$ if $ |f| < f_c$, $0$ otherwise, which selects frequencies below a cut-off frequency $f_c$, and cuts higher frequencies.

The DTFT is a function of a continuous variable $f$, thus its computation cannot be performed by a digital computer. However, for finite duration signals, $x_n$, $n\in\{0,\ldots,N-1\}$, there exists an alternative Fourier representation, namely the discrete Fourier transform (DFT), defined as $\hat{x}_m = \sum_{n=0}^{N-1} x_n e^{-j \frac{2 \pi m n}{N} }$, for $m\in\{0,\ldots,N-1\}$.
Note that the DFT is a sequence, rather than a function of the continuous variable $f$. In particular, the $m$-th element $\hat{x}_m$ of the DFT sequence is the $m$-th sample of the DTFT $X(f)$ at frequency $1/N$: $\hat{x}_m=X(m/N)$. A digital computer can perform the entry-wise product of the DFTs $\hat{x}$ and $\hat{h}$ of two sequences $x$ and $h$: $\hat{y}_m=\hat{x}_m\hat{h}_m $.
However, taking the inverse DFT (IDFT) of the sequence $\hat{y}_m$ yields the circular convolution of the sequences $x_n$ and $h_n$ in the time domain: $y'_k =  \sum_{n=0}^{N-1} x_n h_{(k-n)[N]}$, rather than the linear convolution $y_k =  \sum_{n=0}^{N-1} x_n h_{k-n}$ which represents linear filtering. Nevertheless, the linear convolution of finite duration sequences can be emulated by their circular convolution through zero-padding methods  \cite{Oppenheim-1999,Proakis-1992}.
Finally, it should be pointed out that there exist efficient algorithms ($N \log N$ complexity), named Fast Fourier Transform (FFT) algorithms, to compute the DFT of a finite duration sequence.

In summary, linear filtering can be performed as a linear convolution. Linear convolution can be emulated by circular convolution, through zero-padding methods \cite{Oppenheim-1999,Proakis-1992}. The circular convolution of two sequences can be efficiently performed as the entry-wise multiplications of their DFTs. DFT can be efficiently computed by FFT algorithms.
In other words, if one wants to process a discrete-time signal $x$ by a linear time-invariant filter $h$ through the linear convolution $y=h\ast x$, it is more efficient computationally to do step 1-4 below than to directly compute the convolution.
\begin{enumerate}
\item pad $x$ and $h$ with zeros
\item compute the DFTs of the padded $x$ and $h$
\item multiply entry-wise these DFTs to obtain $\hat{y}$ (circular convolution computed in the Fourier domain)
\item take the inverse DFT of $\hat{y}$ to obtain the filtered y (result of the circular convolution in the time domain, emulating the linear convolution)
\end{enumerate}
This is the reason why in this paper, we focus on the circular convolution of two sequences.

%\item The circular convolution of two sequences can be efficiently performed as the entry-wise multiplications of their DFTs. discrete Fourier transforms (DFT): the product in the Fourier domain of the DFTs $\hat(x)$ and $\hat(h)$ of two sequences $x$ and $h$ corresponds, in the time domain (by Inverse DFT), to the circular convolution of the two sequences.
%
%\item  There exist efficient algorithms ($N \log N$ complexity), named Fast Fourier Transform (FFT) algorithms, to compute the DFT of a finite duration sequence.
%
%
%\end{itemize}
%
%In summary, if one wants to process a discrete-time signal $x$ by a linear time-invariant filter $h$ through the linear convolution $y=h\ast x$, it is more efficient computationally to do step 1-4 below than to directly compute the convolution.
%\begin{enumerate}
%\item pad $x$ and $h$ with zeros
%\item compute the DFTs of the padded $x$ and $h$
%\item multiply entry-wise these DFTs to obtain $\hat{y}$ (circular convolution computed in the Fourier domain)
%\item take the inverse DFT of $\hat{y}$ to obtain the filtered y (result of the circular convolution in the time domain, emulating the linear convolution)
%\end{enumerate}







\item Connection with some prior work on k-way marginals.









For the k-way marginals setting, we think of each row of the database as an element of $\{0, 1\}^d$,  i.e., each user has $d$ binary attributes, for example the attributes can be "Male?", "Married", "Lives in CA?" (in this case $d = 3$). We can write the database as a "histogram": a function $f : \{0, 1\}^d \rightarrow \R$, where $f(x_1, ..., x_d)$ gives the number of users with attribute values $x_1, \ldots, x_d$.  In our example $f(0, 1, 1)$ will be the number of married women living in CA.

A k-way marginal is given by a set $S \subset [d]$, $|S| = k$ and is a function $g_S : \{0, 1\}^S \rightarrow \R$. For each setting of the k attributes in $S$, $g_S$ gives the total number of users in the database that have the corresponding attribute values. For the example, a 2-way marginal is $g_{1, 3}(1, 1)$ which gives the number of men (both married and unmarried) living in CA.

There is some prior work in \url{http://research.microsoft.com/pubs/64344/contingency.pdf} that uses the Fourier transform to compute k-way marginals with less error than the naive approach (and to achieve consistent marginals). I was aware of that but I was not realizing that they actually compute a convolution and the function they are convolving with is sparse. What I mean is:

\begin{itemize}
\item We can extend $g_S$ from the domain $\{0, 1\}^S$ to the domain $\{0, 1\}^d$ in the natural way: components not in $S$ are just ignored (this is more for technical reasons); for example, above we can write $g_{1, 3}(1, 0, 1) = g_{1, 3}(1, 1, 1) = g_{1, 3}(1, 1)$
\item Then we can write $g_S$ as a convolution of $f$ and a function $h_S:\{0, 1\}^d \rightarrow \R$. We define $h_S$ as $h_S(x) = 1$ if and only if $x_i = 0 \:\: \forall i \in S$. The convolution is in the group $(\Z_2)^d$: $(f * h)(x) \triangleq \sum_{z \in \Z_2^d} { f(y + z \mod 2)h(z) }$ (as opposed to $\Z_n$ which is what we have been thinking about, but that does not affect any of the math). We have $(f * h_S)(x) = \sum_{y \mbox{ agrees with} x \mbox{ on } S}{ f(y) }$
\item The function $h_S$ has only $2^k$ nonzero Fourier coefficients (out of $2^d$ total).
\end{itemize}

So, the results in Barak et al. are a special case of computing convolutions of a private function/vector and a public function/vector which is sparse in the Fourier basis.

It seems that in their work, looking at the Fourier basis helps only with $\eps$-differential privacy, but not with $(\eps, \delta)$-d.p. It also seems to help make the marginals consistent.

But I still think it will be interesting to look at functions $h: \Z_2^d \rightarrow \{0, 1\}$ which are approximately sparse in the Fourier domain and see if convolutions $f * h$ for such functions are meaningful/interesting. Might lead to nice applications.


There is work, esp. in learning theory, on analyzing the fourier spectrum of functions $h:\{0, 1\}^d \rightarrow \{0, 1\}$ and proving that certain interesting examples have most of their weight concentrated on a few fourier coefficients (so they are approximately sparse as opposed to exactly sparse, like in Barak et al.). Here the fourier transform I am talking about is the one for $(\Z_2)^d$.


\end{itemize}





Challenge

Can applying differential privacy in the Fourier domain, rather than the time domain, result in an improved privacy-accuracy trade-off?








\subsection{Contributions}


Ongoing work

Randomized response, output perturbation in the time domain, and output perturbation in the Fourier domain: No gain so far
	$\Rightarrow$ noise variance scales with energy of the convolution filter impulse response

Investigating assumptions on convolution filer impulse response (e.g. compressibility) to obtain improved privacy-accuracy trade-off

\begin{table}\label{tab:MSEcomparison}
\begin{tabular}{| l || c | c | c |}
\hline
                                    & \textbf{Linear map $\bA$}  & \textbf{Convolution $\bH$}  & \textbf{p-Compressible Convolution }  \\ \hline \hline
\textbf{UB Output Pert. in time}    &                            &                             &                                     \\ \hline
\textbf{UB  Output Pert. in freq.}  &                            &                             &                                     \\ \hline
\textbf{UB  Input Pert.}            &                            &                             &                                     \\ \hline
\textbf{UB  Iterative algo}         &                            &                             &                                     \\ \hline
\textbf{LB  }                       &                            &                             &                                     \\
\hline
\end{tabular}
\caption{Mean square error for $\ell_1$ neighbors}
\end{table}





\subsection{Prior Work}

Optimizing Linear Counting Queries Under Differential Privacy

http://www.cs.cornell.edu/~mhay/papers/li2010optimizing.pdf

On the Geometry of Differential Privacy

http://research.microsoft.com/apps/pubs/default.aspx?id=119027.

Alex: I am wondering if their results imply that their K-norm mechanism gives optimal bounds for total l2 noise for epsilon-d.p. algorithms (assuming the slicing conjecture).

Haitham Hassanieh, Piotr Indyk, Dina Katabi, and Eric Price "Simple and Practical Algorithm for Sparse Fourier Transform," SODA, 2012.

http://nms.lcs.mit.edu/~dina/pub/soda12.pdf



==> Intron.tex <==
\section{Introduction}
We study the classical convolution. 
Let $x=\{x_0,\ldots,x_{N-1}\}$ be a real input sequence of length $N$, and $h=\{h_0,\ldots,h_{N-1}\}$ a
sequence of length $N$.
The convolution of $x$ and $h$, denoted, $conv(h,x)$, is the sequence $y= x \ast h$ of length $N$ defined by
\begin{equation}\label{eq:circConv}
y_k =  \sum_{n=0}^{N-1} x_n h_{(k-n)[N]}\mbox{, } \forall k\in\{0,\ldots, N-1\}.
\end{equation}
Define the column vectors $\bx=[x_0,\ldots,x_{N-1}]^T \in \R^N$, and $\by=[y_0,\ldots,y_{N-1}]^T \in \R^N$.  The circular convolution (\ref{eq:circConv}) can be written in matrix notation
\begin{equation}\label{eq:MatCircConv}
\by = \bH \bx.
\end{equation}



==> LowerBounds.tex <==
\section{Lower Bounds}

In this section we establish lower bounds for privately approximating
convolutions $\vec{h} \ast \vec{x}$.  For any particular $\vec{h}$, we
derive a lower bound that depends on the Fourier coefficients of
$\vec{h}$. We start with a useful lemma that shows that reconstruction
implies lack of privacy.

\begin{lemma}[\cite{De2011}]
  \label{lm:non-priv-dp}
  Let $\alg$ be an algorithm such that for some $N$ there
  exists a (not necessarily efficient) algorithm $\mathcal{B}$ such that
  \begin{equation*}
    \forall \vec{x} \in \{0, 1\}^N: \Pr[\|\mathcal{B}(\alg(\vec{x})) -
    \vec{x}\|_1 >  \alpha n ] < \beta.
  \end{equation*}
  Then there exist $\eps = \eps(\alpha, \beta)$ and $\delta =
  \delta(\alpha, \beta)$ such that $\alg$ is not $(\eps,
  \delta)$-differentially private.
\end{lemma}

The following lemma is implicit in the foundational work of Dinur and
Nissim. Here we include a full proof for completeness
\begin{lemma}
  \label{lm:DN-lb}
  Let $\vec{A}$ be an $M \times N$ complex matrix with smallest
  (in absolute value) singular value $\lambda_{\min}$. Let $\alg$ be an algorithm that
  for some $M \times N$ matrix $\vec{A}$ and all $\vec{x} \in \{0,
  1\}^N$ satisfies
  \begin{equation*}
    \E[\|\alg(\vec{x}) - \vec{Ax}\|_2^2] <
   \frac{\lambda_{\min}^2\alpha^2N}{8}. 
  \end{equation*}
  Then there exist $\eps = \eps(\alpha, 1/2)$ and $\delta =
  \delta(\alpha, 1/2)$, such that $\alg$ is not $(\eps,
  \delta)$-differentially private.
\end{lemma}
\begin{proof}
  The proof is via the standard Dinur-Nissim attack. We will show
  an algorithm $\mathcal{B}$ that, given $\alg(\vec{x})$ satisfying
  the conditions of the lemma, outputs a vector $\vec{x}'$ such that
  $\|\vec{x} - \vec{x}'\|_1 < \alpha N$ with probability at least
  1/2. Then the lemma follows form Lemma~\ref{lm:non-priv-dp}.

  The algorithm $\mathcal{B}$ outputs an arbitrary (say first in
  lexigraphic order) $\vec{x}' \in \{0, 1\}^N$ such that $\|\vec{Ax}'
  - \alg(\vec{x})\|_2^2 \leq \frac{\lambda_{\min}^2\alpha^2N}{4}$. Let
  us assume for contradiction that some such $\vec{x}'$ satisfies
  $\|\vec{x} - \vec{x}'\|_1 \geq \alpha N$. By Markov's inequality,
  with probability at least 1/2, $\|\alg(\vec{x}) - \vec{Ax}\|^2_2 <
  \frac{\lambda_{\min}^2\alpha^2N}{4}$. Therefore, by the triangle
  inequality, with probability at least 1/2,
  \begin{equation*}
    \|\vec{A}(\vec{x - x}')\|_2^2 \leq (\|\vec{Ax}'  - \alg(\vec{x})\|_2 +
    \|\alg(\vec{x}) - \vec{Ax}\|_2)^2 <  \lambda_{\min}^2\alpha^2N. 
  \end{equation*}
  Since $\|\vec{x - x}'\|_1 \geq \alpha N$ by assumption, $\|\vec{x -
    x}'\|_2^2 \geq \alpha^2N$. Then, by the variational
  characterization of singular values, $\|\vec{A}(\vec{x - x}')\|_2^2
  \geq \alpha^2{N}\lambda^2_{\min}$, a contradiction.
\end{proof}

Assume that we are given a vector $\vec{h} \in \R^N$ such that
$|\hat{h}_1| \geq |\hat{h}_2| \geq \ldots
|\hat{h}_N|$. Lemma~\ref{lm:DN-lb} implies that for some fixed
constant $\eps$ and $\delta$, no $(\eps, \delta)$-differentially
private algorithm can achieve mean squared error $o(|\hat{h}_N|^2N)$,
since the smallest singular value of the corresponding convolution
matrix $\bH$ is $\sqrt{N}\hat{h}_N$. We exploit higher singular values
by restricting $\vec{x}$ to a subspace of the domain of $\bH$. We
first show how to use an algorithm for approximating $\vec{A}\vec{x}$
to approximate a linear map which is a restriction of $\vec{A}$ to
some subspace.

\begin{lemma}
  Let $\alg$ be an $(\eps, \delta)$-differentially private algorithm
  for $\ell_1$ neighbors. Let also $\vec{U}$ be a $N \times K$
  complex matrix whose columns form an orthonormal basis for some
  subspace of $\C^N$. Then an algorithm $\mathcal{B}$ which on input
  $\vec{x} \in \R^K$ outputs $\mathcal{B}(\vec{x}) =
  \alg(\frac{1}{\sqrt{N}}\vec{Ux})$ is $(\eps,
  \delta)$-differentially private for $\ell_1$ neighbors.
\end{lemma}
\begin{proof}
  For any $\vec{x} \in \R^K$ and any measurable subset of the output
  range of $\mathcal{B}$ (which is a subset of the output range of
  $\alg$), we have $\Pr[\mathcal{B}(\vec{x}) \in S] =
  \Pr[\alg(\frac{1}{\sqrt{N}}\vec{Ux}) \in S]$. Therefore, to verify
    that $\mathcal{B}$ satisfies $(\eps, \delta)$-differential
    privacy, we need to verify that for any $\vec{x}, \vec{x}' \in
    \R^K$ such that $\|\vec{x} - \vec{x}'\|_1 \leq 1$ the inequality
    $\|\frac{1}{\sqrt{N}}\vec{U(x - x')}\|_1 \leq 1$ holds. We have
    \begin{equation*}
      \|\frac{1}{\sqrt{N}}\vec{U(x - x')}\|_1 \leq  \|\vec{U(x -
        x')}\|_2 = \|\vec{x - x'}\|_2 \leq \|\vec{x - x'}\|_1 \leq 1. 
    \end{equation*}
    The first and third inequalities hold by H\"{o}lder's
    inequality. The equality holds because the columns of $U$ are unit
    length and mutually orthogonal.
\end{proof}

\begin{theorem}
  \label{thm:main-lb}
  Let $\vec{h} \in \R^N$ be an arbitrary real vector and let us
  relabel the Fourier coefficients of $\vec{h}$ so that $|\hat{h}_1|
  \geq |\hat{h}_2| \geq \ldots |\hat{h}_N|$. There exist fixed
  constant $\eps$ and $\delta > 0$ such that the expected mean squared
  error $\sigma_z$ of any $(\eps, \delta)$-differentially private
  algorithm $\alg$ is at least
  \begin{equation*}
    \sigma_z = \Omega(\max_{K = 1}^N{\frac{K}{N}\hat{h}^2_K}. 
  \end{equation*}
\end{theorem}
\begin{proof}
  We will show that for any constant $\alpha > 0$ and for any $K \in
  [N]$ and for any $(\eps, \delta)$-differentially private algorithm
  where $\eps = \eps(\alpha, 1/2)$ and $\delta = \delta(\alpha, 1/2)$,
  we have $\sigma_z = \Omega(K\hat{h}_K)$. 

  Let $\bF_{[K]}$ be the submatrix of $\bF_N$ whose rows are the
  Fourier basis vectors corresponding to $\hat{h}_1, \ldots,
  \hat{h}_K$ and let $\hat{\bH}_{[K]}$ be the submatrix of $\hat{\bH}$
  consisting of those columns of $\hat{\bH}$ that contain $\sqrt{N}\hat{h}_1,
  \ldots, \sqrt{N}\hat{h}_K$. Consider the matrix $\vec{A} = \frac{1}{\sqrt{N}}
  \bH\bF^H_{[K]}$. Since $\bH = \bF^H\hat{\bH}\bF$, we have
  \begin{equation*}
    \vec{A} = \frac{1}{\sqrt{N}} \bF^H\hat{\bH}\bF\bF^H_{[K]} =
    \frac{1}{\sqrt{N}} \bF^H\hat{\bH}\bF\bI_{[K]} = 
    \bF^H(\frac{1}{\sqrt{N}} \hat{\bH}_{[K]})\bI_K, 
  \end{equation*}
  where $\bI_{[K]}$ is a $N \times K$ matrix with 1's on the
  diagonal. This is a singular value decomposition of $\vec{A}$, and
  therefore the singular values of $\vec{A}$ are the diagonal entries
  of $\frac{1}{\sqrt{N}} \hat{\bH}_{[K]}$, i.e.~$\hat{h}_1,
  \ldots, \hat{h}_K$.

  By Lemma~\ref{lm:DN-lb}, any $(\eps, \delta)$-differentially private
  algorithm $\mathcal{B}$ satisfies for some $\vec{x} \in \R^K$
  \begin{equation*}
    \E[\|\mathcal{B}(\vec{x}) - \vec{Ax}\|_2^2] = \Omega(KN|\hat{h}_K|^2). 
  \end{equation*}
  In particular, this holds for the algorithm $\mathcal{B}$ of
  Lemma~\ref{lm:subspace}. The proof is completed by observing that
  $\E[\|\mathcal{B}(\vec{x}) - \vec{Ax}\|_2^2] = N\sigma_z$. 
\end{proof}


==> OutputPerturbation.tex <==
\subsection{Output Perturbation}



\subsubsection{Time Domain}


%---------------------------
% $(\eps,0)$- diff privacy
%---------------------------

\begin{theorem}[$OPT$]\label{thm:OPT}
Consider the linear map $\by=\bA \bx$, where $\bA \in \R^{M \times N}$. Suppose that on input $\bx$ algorithm $\alg_{OPT}$ outputs   $\tilde{\by}=\bA \bx + \bz$, where $\bz$ is sampled from $\R^M$ with probability density $\alpha_{q, \eps, \|\bA \|_{p,q}}(\R^M)\mu_{q, \eps, \|\bA \|_{p,q}}(\vec{z})$, then $\alg_{OPT}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors,  unbiased, and it achieves MSE
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{ll}
 2 \frac{\|\bA\|_1^2}{\eps^2}  & \mbox{ if } p=1  \\%\mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
 \left(1 + \frac{1}{M} \right) M \frac{\|\bA\|_2^2 }{\eps^2} & \mbox{ if } p=2 \\ %\mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
\end{array}
\right.
\end{equation}
\end{theorem}

\begin{proof}
The algorithm $\alg_{OPT}$ is $(\eps,0)$-differentially private by Theorem~\ref{th:eps0-DiffPriv} and Lemma~\ref{lm:spqSensitivity}. The MSE for $p=1$ comes from the fact that $\bz$ is sampled from $\Lap(0, \|\bA\|_1/\eps)^M$, and for $p=2$ from Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity}).
\end{proof}

\begin{cor}
Consider the circular convolution $\bH \in \R^{N \times N}$ {\rm (\ref{eq:circConv})}. The algorithm $\alg_{OPT}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{ll}
 2 \frac{\|\bh\|_1^2}{\eps^2}  & \mbox{ if } p=1    \\
 \left(1 + \frac{1}{N} \right) N^2\frac{\max_{m} |\hat{h}_m|^2 }{\eps^2} & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
\end{cor}

\begin{proof}
Applying Theorem~\ref{thm:OPT} to the circular convolution $\bH$ {\rm (\ref{eq:circConv})}, and using Lemma~\ref{lm:DiagConvNorm} yields the results.
\end{proof}

Note that
$
 \frac{\|\bh\|_1^2}{\eps^2}
\leq  N^2 \frac{\max_{m} |\hat{h}_m|^2}{\eps^2}
\leq  N\frac{\|\bh\|_1^2 }{\eps^2}.
$
The first inequality implies that guaranteeing differential privacy for $\ell_1$ neighbors requires less noise than for $\ell_2$ neighbors.

%------------------------------
% $(\eps,delta)$- diff privacy
%------------------------------

\begin{theorem}[$\delta-OPT$]\label{thm:deltaOPT}
Consider the linear map $\by=\bA \bx$, where $\bA \in \R^{M \times N}$. Suppose that on input $\bx$ algorithm $\alg_{\delta OPT}$ outputs   $\tilde{\by}=\bA \bx + \bz$, where $z_m$ is sampled from $\R$ with probability density $\Lap(0, \|\bA_{m:}\|_p/\eps_m)$, with $\eps_m = \frac{\eps}{\sqrt{2M \ln (1/\delta)}}$. Then $\alg_{\delta OPT}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors,  unbiased, and it achieves MSE on the $m$-th entry
\begin{equation}
\sigma_{z_m}^2=
 4 M \frac{\|\bA_{m:}\|_p^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)
\end{equation}
\end{theorem}

\begin{proof}
The proof follows from Theorems~\ref{th:eps0-DiffPriv} and~\ref{thm:fancy-comp}.
\end{proof}

\begin{cor}
Consider the circular convolution $\bH \in \R^{N \times N}$ {\rm (\ref{eq:circConv})}. The algorithm $\alg_{\delta OPT}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{ll}
 4 N \frac{\|\bh\|_{\infty}^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)  & \mbox{ if } p=1    \\
 4 N \frac{\|\bh\|_2^2}{\eps^2} \ln\left(\frac{1}{\delta}\right) & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
\end{cor}

%Output perturbation in the time domain by additive noise
%\begin{equation}
%\tilde{\by}=\by + \bz = \bA \bx + \bz,
%\end{equation}
%where $\bz$ is a random noise vector in $\R^N$.
%%
%If $\bz$ is sampled with probability density $\alpha_{q, \eps, \|\bA \|_{p,q}}(\R^N)\mu_{q, \eps, \|\bA \|_{p,q}}(\vec{z})$, then by Theorem~\ref{th:eps0-DiffPriv}, $\tilde{\by}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors.
%%
%Each noise component $z_n$, $n \in \{0,\ldots,N-1\}$ has mean zero, and variance
%\begin{equation}
%\sigma_z^2= \E [|z_n|^2]=
%\left\{
%\begin{array}{lll}
% 2 \frac{\|\bA\|_1^2}{\eps^2}  & \mbox{ if } p=1 & \mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
% \left(1 + \frac{1}{N} \right) \frac{N \|\bA\|_2^2 }{\eps^2} & \mbox{ if } p=2 & \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
%\end{array}
%\right.
%\end{equation}

%In the case of a circular convolution matrix $\bA=\bH$,
%\begin{equation}
%\sigma_z^2= \E [|z_n|^2]=
%\left\{
%\begin{array}{lll}
% 2 \frac{\|\bh\|_1^2}{\eps^2}  & \mbox{ if } p=1 & \mbox{ by Eq. (\ref{eq:Hnorms})} \\
% \left(1 + \frac{1}{N} \right) N^2\frac{\max_{m} |\hat{h}_m|^2 }{\eps^2} & \mbox{ if } p=2 & \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:Hnorms})}
%\end{array}
%\right.
%\end{equation}




%\subsection{Frequency (Fourier) Domain}
\subsubsection{Transform Domain}

\begin{theorem}[$OPF$]\label{thm:OPF}
Consider the linear map $\by=\bA \bx$, where $\bA \in \R^{M \times N}$ has decomposition $\bA = \bU \bD \bV^H$, with $\bD \in \C^{M \times N}$ diagonal, and $\bU\in\C^{M \times M}$ and $\bV\in\C^{N \times N}$ unitary. This could be the singular value decomposition, or eigen-decomposition $\bA = \bU \bD \bU^H$ if $\bA$ is normal ($\bA \bA^H=\bA^H \bA$).

Suppose that on input $\bx$ algorithm $\alg_{OPF}$ first adds noise in the transform domain: $\check{\by}= \bU^H \by + \bz$, where $\bz$ is sampled from $\alpha_{q, \eps, \| \bD \bV^H \|_{p,q}}(\C^N)\mu_{q, \eps, \|\bD \bV^H \|_{p,q}}(\vec{z})$, and then outputs   $\tilde{\by}= \bU \check{\by}$.
Then $\alg_{OPF}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, unbiased and it achieves MSE
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{ll}
 2 \frac{\|\bD \bV^H\|_1^2}{\eps^2}  & \mbox{ if } p=1 \\ %& \mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
 \left(1 + \frac{1}{M} \right) M \frac{ \|\bA\|_{2}^2 }{\eps^2}  & \mbox{ if } p=2. \\ %& \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
\end{array}
\right.
\end{equation}
\end{theorem}

\begin{proof}

In the transform domain $\bU$, the linear map $\by = \bA \bx$ becomes $\hat{\by}= \bU^H \by = \bD \bV^H \bx$. Then $\check{\by}= \hat{\by} + \bz=\bD \bV^H \bx + \bz$. If $\bz$ is sampled from $\alpha_{q, \eps, \| \bD \bV^H \|_{p,q}}(\C^N)\mu_{q, \eps, \|\bD \bV^H \|_{p,q}}(\vec{z})$, then by Theorem~\ref{th:eps0-DiffPriv}, $\check{\by}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, and consequently, $\tilde{\by}=\bU \check{\by}$ is also $(\eps,0)$-differentially private by Theorem~\ref{thm:simple-composition}.
%
%For $p=2$, note that $\|\bD \bV^H\|_{2}= \|\bD\|_{2} = \|\bA\|_{2}$ since $\bV^H$ is a unitary matrix. For $p=1$,
%$  \|\bD \bV^H\|_{1}= \max_{n\in[N]} \sum_{m=1}^{M} \sigma_m |v_{m n}|$.
%
Regarding the MSE, note that the output of $\alg_{OPF}$ is $\tilde{\by}= \by + \bU \bz$. The final noise $\bz'= \bU \bz$ has mean 0, and the same covariance matrix as $\bz$.
Thus, the MSE is
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{lll}
 2 \frac{\|\bD \bV^H\|_1^2}{\eps^2}  & \mbox{ if } p=1 & \mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
 \left(1 + \frac{1}{M} \right) M \frac{ \|\bD \bV^H\|_{2} }{\eps^2}= \left(1 + \frac{1}{M} \right) M \frac{ \|\bA\|_{2}^2 }{\eps^2}   & \mbox{ if } p=2 & \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
\end{array}
\right.
\end{equation}

\end{proof}



\begin{cor}
Consider the circular convolution $\bH =\bF_N^{H} \hat{\bH}\bF_N $ {\rm (\ref{eq:circConv})}. The algorithm $\alg_{OPF}$ in the Fourier domain $\bU=\bF_N^{H}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{ll}
 2 \frac{\| \hat{\bh}\|_1^2}{\eps^2}  & \mbox{ if } p=1  \\
 \left(1 + \frac{1}{N} \right) N^2\frac{\max_{m} |\hat{h}_m|^2 }{\eps^2}  & \mbox{ if } p=2.
\end{array}
\right.
\end{equation}
\end{cor}

For $p=2$, output perturbation in the time or the transform domain results in the same MSE. However, for $p=1$, the difference in MSE depends on how $\|\bh\|_1$ and $\|\hat{\bh}\|_1$ relate to one another. In general, we know that  $\frac{1}{\sqrt{N}}\|\bh\|_1 \leq \|\hat{\bh}\|_1 \leq N \|\bh\|_1$.


%------------------------------
% $(\eps,delta)$- diff privacy
%------------------------------

\begin{theorem}[$\delta-OPF$]\label{thm:deltaOPF}
Consider the linear map $\by=\bA \bx$, where $\bA \in \R^{M \times N}$ has decomposition $\bA = \bU \bD \bV^H$. Suppose that on input $\bx$ algorithm $\alg_{\delta OPF}$ first adds noise in the transform domain: $\check{\by}= \bU^H \by + \bz$,  where $z_m$ is sampled from $\Lap(0, |d_m| \|\bV^H_{m:}\|_p/\eps_m)$, with $\eps_m = \frac{\eps}{\sqrt{2M \ln (1/\delta)}}$, and then outputs  $\tilde{\by}= \bU \check{\by}$. Then $\alg_{\delta OPF}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors,  unbiased, and it achieves MSE on the $m$-th entry
\begin{equation}
\sigma_{z_m}^2=
 4 M \frac{|d_m|^2 \|\bV^H_{m:}\|_p^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)
\end{equation}
\end{theorem}

\begin{cor}
Consider the circular convolution $\bH =\bF_N^{H} \hat{\bH}\bF_N $ {\rm (\ref{eq:circConv})}. The algorithm $\alg_{\delta OPF}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE on the $m$-th entry
\begin{equation}
\sigma_{z_n}^2=
\left\{
\begin{array}{ll}
 4 N \frac{|\hat{h}_m|^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)  & \mbox{ if } p=1    \\
 4 N^2 \frac{|\hat{h}_m|^2}{\eps^2} \ln\left(\frac{1}{\delta}\right) & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
Thus, the average MSE per entry is
\begin{equation}
\sigma_{z}^2=
\left\{
\begin{array}{ll}
 4 \frac{\|\bh\|_2^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)  & \mbox{ if } p=1    \\
 4 N \frac{\|\bh\|_2^2}{\eps^2} \ln\left(\frac{1}{\delta}\right) & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
\end{cor}

For $p=1$, output perturbation in the Fourier domain yields a lower MSE as $\|\bh\|_2^2 \leq N \|\bh\|_{\infty}^2$. For $p=2$, output perturbation in the time or the transform domain results in the same MSE.

%\junk{
%The noise $\bz'$ has mean zero, and covariance matrix
%\begin{equation}
%\E [\bz' \bz'^T]=
%\left\{
%\begin{array}{lll}
% 2 \frac{\|\bD \bV^H\|_1^2}{\eps^2} \bI_N & \mbox{ if } p=1 & \mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
% \left(1 + \frac{1}{N} \right) \frac{N \|\bA\|_{2}^2 }{\eps^2} \bI_N  & \mbox{ if } p=2 & \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
%\end{array}
%\right.
%\end{equation}
%}

%Let $\bA = \bU \bD \bV^H$ denote a singular value decomposition (SVD) of $\bA \in \R^{M \times N}$ , where $\bD$ is an $M \times N$ diagonal matrix whose diagonal entries are in descending order, and $\bU$ and $\bV$ are unitary $M \times M$ and $N \times N$ matrices respectively. (If $\bA$ is a normal matrix, i.e. a square $N \times N$ matrix such that $\bA \bA^H=\bA^H \bA$, then its eigen-decomposition $\bA = \bU \bD \bU^H$ in a unitary basis $\bU \in \C^{N \times N}$ can  be used instead of the SVD.)
%Output perturbation in the singular space by additive noise
%\begin{equation}
%\begin{split}
%\tilde{\hat{\by}}&= \hat{\by} + \bz' = \bD \bV^H \bx + \bz' \\
%\tilde{\by}&= \bU \tilde{\hat{\by}} =  \bA  \bx + \bU \bz' = \by + \bz,
%\end{split}
%\end{equation}
%where $\bz'$ is a random noise vector in $\C^N$.
%
%If $\bz'$ is sampled with probability density $\alpha_{q, \eps, \| \bD \bV^H \|_{p,q}}(\C^N)\mu_{q, \eps, \|\bD \bV^H \|_{p,q}}(\vec{z})$, then by Theorem~\ref{th:eps0-DiffPriv}, $\tilde{\hat{\by}}$ is $(\eps,0)$-differentially private for $\ell_p$ neighbors, and consequently, $\tilde{\by}$ is also $(\eps,0)$-differentially private by Lemma~\ref{}.
%In the case of a circular convolution matrix $\bA=\bH$,
%\begin{equation}
%\sigma_z^2=
%\left\{
%\begin{array}{lll}
% 2 \frac{\| \hat{\bh}\|_1^2}{\eps^2}  & \mbox{ if } p=1 & \mbox{ by Eq. (\ref{eq:pqsensitivity})} \\
% \left(1 + \frac{1}{N} \right) N^2\frac{\max_{m} |\hat{\bh}_m|^2 }{\eps^2}  & \mbox{ if } p=2 & \mbox{ by Lemma~\ref{lm:l2-covar} and Eq. (\ref{eq:pqsensitivity})}
%\end{array}
%\right.
%\end{equation}


==> Preliminaries.tex <==
\subsection{Preliminaries}

The $p$-norm of a column vector $\bx=[x_0,\ldots,x_{N-1}]^T \in \C^N$ is defined by
%\begin{equation}\label{eq:p-norm}
$
\| \bx \|_p = \left( \sum_{n=0}^{N-1} |x_n|^p\right)^{\frac{1}{p}}.
$
%\end{equation}

\begin{definition}
The $(p,q)$-operator norm of a matrix $\bA \in \C^{M\times N}$ induced by the p-norm in the input vector space $\C^N$ and the q-norm in the output vector space $\C^M$ is defined by
\begin{equation}\label{eq:operatorNorm}
\| \bA \|_{p,q} = \max_{\bx : \|\bx\|_p=1}  \| \bA \bx \|_q.
%= \max_{\bx \neq \b0} \frac{\| \bA \bx \|_q}{\| \bx \|_p}
\end{equation}
In particular, denoting $\|\bA\|_{p,p}=\|\bA\|_p$,
\begin{equation}
\begin{split}
\| \bA \|_1 &= \max_{n\in[N]} \|\bA_{:n}\|_1 =  \max_{n\in[N]} \sum_{m=1}^{M} |a_{mn}|, \qquad  \mbox{ largest 1-norm of the columns }  \{\bA_{:n}\}_{n\in[N]} \\
\| \bA \|_2 &= \max_{n\in[N]} \sigma_n(\bA) =  \max_{n\in[\min(M,N)]} \sqrt{\lambda_n(\bA^H \bA)}, \qquad  \mbox{spectral norm (largest singular value) }\\
\| \bA \|_{\infty} &= \max_{m\in[M]} \|\bA_{m:}^H\|_1 =  \max_{m\in[M]} \sum_{n=1}^{N} |a_{mn}|, \qquad  \mbox{ largest 1-norm of the rows } 
%\| \bU \bA \bV \|_2&= \| \bA \|_2, \quad  \forall \mbox{ unitary } \bU, \: \bV  \mbox{ : unitarily invariant norm}
\end{split}
\end{equation}
Note that the 2-operator norm is unitarily invariant: $\| \bA \|_2 =\| \bU \bA \bV \|_2, \quad \forall \mbox{ unitary } \bU, \: \bV$.
%\begin{itemize}
%\item
%$\|\bA\|_1$ is the largest 1-norm of the columns $\{\bA_{:n}\}_{n\in[N]}$ of $\bA$
%\begin{equation}
%\| \bA \|_1 = \max_{n\in[N]} \|\bA_{:n}\|_1 =  \max_{n\in[N]} \sum_{m=1}^{M} |a_{mn}|
%\end{equation}
%\item $\|\bA\|_2$ is the spectral norm (largest singular value), which is unitarily invariant
%\begin{equation}
%\begin{split}
%\| \bA \|_2 &= \max_{n\in[N]} \sigma_n(\bA) =  \max_{n\in[N]} \sqrt{\lambda_n(\bA^H \bA)}\\
%\| \bU \bA \bV \|_2 &= \| \bA \|_2, \mbox{ for any two unitary matrices } \bU \mbox{ and } \bV.\\
%\end{split}
%\end{equation}
%\end{itemize}
\end{definition}


%If $p=q$, we will denote $\|\bA\|_{p,p}=\|\bA\|_p$.
%
\begin{lemma}
Let $\bA \in \C^{M\times N}$ and $\bx \in \C^N$. Then
$\| \bA \bx \|_q \leq \| \bA \|_{p,q} \| \bx \|_p$.
\end{lemma}
%
\junk{
In particular, if $p=q$, the operator norm  $\| \bA \|_{p,p}=\| \bA \|_p$ is a sub-multiplicative norm: For any two matrices $\bA$ and $\bB$ in $\R^N$,
\begin{equation}\label{eq:submult}
\| \bA \bB \|_p \leq \| \bA \|_p  \| \bB \|_p.
\end{equation}
}

%\begin{lemma}
%Let $\bA \in \C^{M\times N}$. Then
%\begin{itemize}
%\item
%$\|\bA\|_1$ is the largest 1-norm of the columns $\{\bA_{:n}\}_{n\in[N]}$ of $\bA$
%\begin{equation}
%\| \bA \|_1 = \max_{n\in[N]} \|\bA_{:n}\|_1 =  \max_{n\in[N]} \sum_{m=1}^{M} |a_{mn}|
%\end{equation}
%\item $\|\bA\|_2$ is the spectral norm (largest singular value), which is unitarily invariant
%\begin{equation}
%\begin{split}
%\| \bA \|_2 &= \max_{n\in[N]} \sigma_n(\bA) =  \max_{n\in[N]} \sqrt{\lambda_n(\bA^H \bA)}\\
%\| \bU \bA \bV \|_2 &= \| \bA \|_2, \mbox{ for any two unitary matrices } \bU \mbox{ and } \bV.\\
%\end{split}
%\end{equation}
%\end{itemize}
%
%\end{lemma}

%If $p=q=1$, then $\|\bA\|_1$ is the largest 1-norm of the columns $\{\bA_{:n}\}_{n\in[N]}$ of $\bA$.
%\begin{equation}
%\| \bA \|_1 = \max_{n\in[N]} \|\bA_{:n}\|_1 =  \max_{n\in[N]} \sum_{m=1}^{M} |a_{mn}|
%\end{equation}
%
%If $p=q=2$, then $\|\bA\|_2$ is the spectral norm (largest singular value), which is unitarily invariant
%\begin{equation}
%\begin{split}
%\| \bA \|_2 &= \max_{n\in[N]} \sigma_n(\bA) =  \max_{n\in[N]} \sqrt{\lambda_n(\bA^H \bA)}\\
%\| \bU \bA \bV \|_2 &= \| \bA \|_2 \mbox{ for any two unitary matrices } \bU \mbox{ and } \bV.\\
%\end{split}
%\end{equation}

\junk{
If $p=q=\infty$, then $\|\bA\|_{\infty}$ is the largest 1-norm of the rows $\{\bA_{m:}\}_{m\in[M]}$ of $\bA$.
\begin{equation}
\| \bA \|_{\infty} = \max_{m\in[M]} \|\bA_{m:}\|_1 =  \max_{m\in[M]} \sum_{n=1}^{N} |a_{mn}|
\end{equation}
}

\begin{lemma}\label{lm:DiagConvNorm}
If $\bA=\diag(a_1,\ldots,a_N)$ is a diagonal matrix, then
\begin{equation} \label{eq:DiagNorms}
\begin{split}
%\|\bA\|_1 & = \|\bA\|_2 =  \max_{m} |a_m|
\|\bA\|_1 & = \|\bA\|_2 = \|\bA\|_{\infty} =  \max_{m} |a_m|
\end{split}
\end{equation}
If $\bH$ is a circulant matrix {\rm (\ref{eq:circConv})}, then
\begin{equation} \label{eq:Hnorms}
\begin{split}
\|\bH\|_1 & = \|\bH\|_{\infty} = \|\bh\|_1\\
%\|\bH\|_1 & = \|\bh\|_1\\
\|\bH\|_2 & = \max_{m \in \{0\ldots N-1\}} \sqrt{N} |\hat{h}_m|
\end{split}
\end{equation}
\end{lemma}

\begin{lemma}\label{lm:spqSensitivity}
Let $s_{p,q}$ denote the $\ell_q$-sensitivity of the linear map $\bA$ for $\ell_p$-neighbors.
Then,
\begin{equation}\label{eq:pqsensitivity}
s_{p,q} = \max_{\bx,\bx': \|\bx-\bx'\|_p \leq 1} \|\bA (\bx -\bx') \|_q = \|\bA \|_{p,q}
\end{equation}
\end{lemma}



%Indeed, if $\bx$ and $\bx'$ are $\ell_p$ neighbors, then
%\begin{equation}
%\|\by(\bx) - \by(\bx')\|_q = \|\bA (\bx -\bx') \|_q \leq  \|\bA \|_{p,q} \|\bx -\bx'\|_p = \|\bA \|_{p,q}.
%\end{equation} 

==> Roadmap.tex <==
\section{Roadmap}

==> StandardUpperBounds.tex <==
\subsection{Standard Upperbounds}\label{sec:StdUB}

In this section, we first derive bounds on the MSE of $(\eps,0)$- and $(\eps,\delta)$-differentially private algorithms for linear maps based on input and output perturbation techniques. Then we apply these bounds to the particular case of circular convolution. These bounds will be used as a benchmark to compare the algorithm proposed in Section~\ref{sec:compressibleFilter}.

%\input{Preliminaries}
%
%\input{OutputPerturbation}
%
%\input{InputPerturbation}

\subsubsection{Output Perturbation in Time Domain}


\begin{theorem}[$\delta-OT$]\label{thm:deltaOT-conv}
Consider the circular convolution $\bH \in \R^{N \times N}$ {\rm (\ref{eq:circConv})}.
Suppose that on input $\bx$ algorithm $\alg_{\delta OT}$ outputs   $\tilde{\by}=\bH \bx + \bz$, where $z_m$ is sampled from $\R$ with probability density $\Lap(0, \|\bH_{m:}\|_p/\eps_m)$, with $\eps_m = \frac{\eps}{\sqrt{2M \ln (1/\delta)}}$. The algorithm $\alg_{\delta OT}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE
\begin{equation}
\sigma_z^2=
\left\{
\begin{array}{ll}
 4 N \frac{\|\bh\|_{\infty}^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)  & \mbox{ if } p=1    \\
 4 N \frac{\|\bh\|_2^2}{\eps^2} \ln\left(\frac{1}{\delta}\right) & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
\end{theorem}
Guaranteeing differential privacy for $\ell_1$ neighbors requires less noise than for $\ell_2$ neighbors.

\subsubsection{Output Perturbation in Frequency Domain}


\begin{theorem}[$\delta-OF$]\label{thm:deltaOF-conv}
Consider the circular convolution $\bH =\bF_N^{H} \hat{\bH}\bF_N $ {\rm (\ref{eq:circConv})}.
Suppose that on input $\bx$ algorithm $\alg_{\delta OF}$ first adds noise in the Fourier domain: $\check{\by}= \bF_N \by + \bz$,  where $z_m$ is sampled from $\Lap(0, |\sqrt{N} \hat{h}_m| \|\bF_{m:}\|_p/\eps_m)$, with $\eps_m = \frac{\eps}{\sqrt{2M \ln (1/\delta)}}$, and then outputs  $\tilde{\by}= \bF_N^H \check{\by}$.
The algorithm $\alg_{\delta OF}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE on the $m$-th entry
\begin{equation}
\sigma_{z_n}^2=
\left\{
\begin{array}{ll}
 4 N \frac{|\hat{h}_m|^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)  & \mbox{ if } p=1    \\
 4 N^2 \frac{|\hat{h}_m|^2}{\eps^2} \ln\left(\frac{1}{\delta}\right) & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
Thus, the average MSE per entry is
\begin{equation}
\sigma_{z}^2=
\left\{
\begin{array}{ll}
 4 \frac{\|\bh\|_2^2}{\eps^2} \ln\left(\frac{1}{\delta}\right)  & \mbox{ if } p=1    \\
 4 N \frac{\|\bh\|_2^2}{\eps^2} \ln\left(\frac{1}{\delta}\right) & \mbox{ if } p=2
\end{array}
\right.
\end{equation}
\end{theorem}

For $p=1$, output perturbation in the Fourier domain yields a lower MSE than output perturbation in the time domain, as $\|\bh\|_2^2 \leq N \|\bh\|_{\infty}^2$.
For $p=2$, output perturbation in the time or the transform domain results in the same MSE.


\subsubsection{Input Perturbation}


\begin{theorem}[$\delta-IT$]\label{thm:deltaIT-conv}
Consider the circular convolution $\bH \in \R^{N \times N}$ {\rm (\ref{eq:circConv})}.
Suppose that algorithm $\alg_{\delta IT}$ first adds noise to the input in the time domain: $\tilde{\bx}= \bx + \bz$, where $\bz$ is sampled from $\Lap\left(0, \frac{\sqrt{2M \ln (1/\delta)}}{\eps}\right)^M$, and then outputs   $\tilde{\by}= \bH \tilde{\bx}$.
Then the algorithm $\alg_{\delta IPT}$ is $(\eps,\delta)$-differentially private for $\ell_p$ neighbors, unbiased, and achieves MSE
\begin{equation}\label{eq:MSE_deltaIPT-Conv}
\sigma_{z}^2=
 4 N \frac{\| \bh \|_2^2}{\eps^2} \ln \left( \frac{1}{\delta} \right)
\end{equation}

\end{theorem}

==> _region_.tex <==
\message{ !name(CompressibleFIR.tex)}
\message{ !name(CompressibleFIR.tex) !offset(70) }
\begin{equation*}
    \sigma_z^2 \leq C\frac{\log N \log (1/\delta)}{\eps^2} \sum_{k = 1}^{\log
      N}{\frac{1}{2^k}\sum_{i = N/2^k + 1}^{N/2^{k-1}}{|\hat{h}_i|^2}}.
  \end{equation*}
\end{lemma}

\begin{theorem}
  Let $\vec{h}$ be a $(c, 2)$-compressible vector. Then
  Algorithm~\ref{alg:compressible} satisfies $(\eps,
  \delta)$-differential privacy and achieves expected mean squared error
  $O(\frac{c\log^2 N \log (1/\delta)}{N\eps^2})$.
\end{theorem}

\begin{theorem}
  Let $\vec{h}$ be a $(c, p)$-compressible vector for some constant $p
  > 2$. Then Algorithm~\ref{alg:compressible} satisfies $(\eps,
  \delta)$-differential privacy and achieves expected mean squared error
  $O(\frac{c\log N \log (1/\delta)}{N\eps^2})$.
\end{theorem}

\junk{By Theorem~\ref{thm:main-lb}, when $|\hat{h}_1| = c$ and $\eps$,
$\delta$ are sufficiently small constants, any $(\eps,
\delta)$-differentially private algorithm incurs with mean squared
error $\sigma_z = \Omega(\frac{c}{N})$. Therefore,
Algorithm~\ref{alg:compressible} is almost optimal for $(c,
p)$-compressible $\vec{h}$ when $p\geq 2$. }

\begin{theorem}
  For any $\vec{h}$, Algorithm ~\ref{alg:compressible} satisfies $(\eps,
  \delta)$-differential privacy and achieves expected mean squared
  error $O(\specLB(\vec{h})\frac{\log^3N \ln (1/\delta)}{\eps^2})$. 
\end{theorem}
\begin{proof}
  By Lemma~\ref{lm:compr-error}, we know that
  
\message{ !name(CompressibleFIR.tex) !offset(-38) }

